Automated Extraction of Fine-Grained Standardized Product Information from Unstructured Multilingual Web Data

Extracting structured information from unstructured data is one of the key challenges in modern information retrieval applications, including e-commerce. Here, we demonstrate how recent advances in machine learning, combined with a recently published multilingual data set with standardized fine-grained product category information, enable robust product attribute extraction in challenging transfer learning settings. Our models can reliably predict product attributes across online shops, languages, or both. Furthermore, we show that our models can be used to match product taxonomies between online retailers.

==> titelseiten.tex <==
%%
%% Berliner Hochschule für Technik --  Abschlussarbeit
%%
%% Titelseiten und Erklärungen 
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\maketitle
\clearpage
%\thispagestyle{empty}
% Rueckseite (leer)
%% 
~
\newpage

\input{abstract_de.tex}
\input{abstract_en.tex}
\clearpage

\ifthenelse{\boolean{@entwurfset}}
    {

    }
    {
      ~
      \newpage
      \vfill
      \section*{Aufgabenblatt -- durch Original austauschen !!!}
      \vfill
      \clearpage
      ~
      \newpage
    }
\vspace{10ex}
\section*{Erklärung}
Ich  versichere, dass  ich diese  Abschlussarbeit ohne  fremde  Hilfe selbstständig
verfasst und  nur die  angegebenen Quellen und  Hilfsmittel benutzt  habe. Wörtlich
oder dem  Sinn nach  aus anderen  Werken entnommene Stellen  sind unter  Angabe der
Quellen kenntlich gemacht.
\vspace{10ex}\\

\hrule
{\small{Datum}}\hfill{\small{Unterschrift}}


\pagenumbering{roman}
\tableofcontents
\listoffigures



